Reliable Slicing of 5G Transport Networks with Dedicated Protection

In 5G networks, slicing allows partitioning of network resources to meet stringent end-to-end service requirements across multiple network segments, from access to transport. These requirements are shaping technical evolution in each of these segments. In particular, the transport segment is currently evolving in the direction of the so-called elastic optical networks (EONs), a new generation of optical networks supporting a flexible optical-spectrum grid and novel elastic transponder capabilities. In this paper, we focus on the reliability of 5G transport-network slices in EON. Specifically, we consider the problem of slicing 5G transport networks, i.e., establishing virtual networks on 5G transport, while providing dedicated protection. As dedicated protection requires large amount of backup resources, our proposed solution incorporates two techniques to reduce backup resources: (i) bandwidth squeezing, i.e., providing a reduced protection bandwidth with respect to the original request; and (ii) survivable multi-path provisioning. We leverage the capability of EONs to fine tune spectrum allocation and adapt modulation format and Forward Error Correction (FEC) for allocating rightsize spectrum resources to network slices. Our numerical evaluation over realistic case-study network topologies quantifies the spectrum savings achieved by employing EON over traditional fixed-grid optical networks, and provides new insights on the impact of bandwidth squeezing and multi-path provisioning on spectrum utilization.

==> figures/heuristic.tex <==
\section{Heuristic Algorithm}\label{sec:heuristic}

\subsection{Optimal solution for a VLink}\label{sec:single-heuristic}
There are several challenges for solving our problem for a single VLink $\bar{e}$. First, There are combinatorial number of ways to choose at most $q$ paths out of $k$ shortest paths as the prospective lightpaths of a VLink. The possibility of a path being used zero, one, or more than one times in a solution result in a multi-set $(\mathcal{P}_{\bar{e}}^k, m_1)$ where $m_1:\mathcal{P}_{\bar{e}}^k \rightarrow N_q$. Each of the paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$ can, in turn, use different combinations of tuples to achieve the bandwidth demand $\bar{\beta}_{\bar{e}}$, resulting in another multi-set $(\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_2)$, where $(\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)})$ is the set of tuples from $\mathcal{R}$ and $m_2:\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)} \rightarrow N_q$ such that $|(\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_2)| = |(\mathcal{P}_{\bar{e}}^k, m_1)|$. Second, for each $<$path, tuple$>$ pairs, one has to find a multi-set of spectrum slice indices, represented as $(S_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_3)$ such that $|(\mathcal{S}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_3)| = |(\mathcal{P}_{\bar{e}}^k, m_1)|$ where $m_3:S_{\bar{e}(\mathcal{P}_{\bar{e}}^k, m_1)} \rightarrow N_q$, while satisfying constraints \eqn{eq:sl-once} and \eqn{eq:contiguity}. A solution to $\bar{e}$ consists of these three multi-sets represented as $\mathcal{I}_{\bar{e}}=\{(\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_2), ({S}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_3)\}$. However, an optimal solution for $\bar{e}$ denoted by $\mathcal{A}_{\bar{e}}$ is the one that minimizes the number of required spectrum slices. If $\mathcal{M}{(\mathcal{P}_{\bar{e}}^k, m_1)}$, $\mathcal{M}{(\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_2)}$, and $\mathcal{M}{(\mathcal{S}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_3)}$ are the set of all possible multi-sets of $(\mathcal{P}_{\bar{e}}^k, m_1)$, $(\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_2)$, and $(\mathcal{S}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_3)$, respectively, and $n(\mathcal{I}_{\bar{e}})$ denotes the number of required spectrum slices for the solution $\mathcal{I}_{\bar{e}}$, $\mathcal{A}_{\bar{e}}$ can be defined as follows:

%spectrum contiguity and capacity constraints as well as ensuring that a slice on an SLink can be allocated to at most one lightpath

%that consists of three multi-sets defined as $\mathcal{A}_{\bar{e}}=\{(\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{T}_{\bar{e}(\mathcal{P}_{\bar{e}}^k, m_1)}, m_2), (S_{\bar{e}(\mathcal{P}_{\bar{e}}^k, m_1)}, m_3)\}$. An optimal solution $\mathcal{A}_{\bar{e}}$ is the one that requires the minimal number of spectrum slices. In other words, there is no other solution for $\bar{e}$ that requires less number of slices than that of $\mathcal{A}_{\bar{e}}$.

\vspace{-1.0em}
\begin{equation}
\mathcal{A}_{\bar{e}} = \argminA_{\mathcal{I}_{\bar{e}} \in \mathcal{M}{(\mathcal{P}_{\bar{e}}^k, m_1)} \times \mathcal{M}{(\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_2)} \times \mathcal{M}{(\mathcal{S}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_3)}}  n(\mathcal{I}_{\bar{e}}) \label{eq:heu-eq1}
\end{equation}
\vspace{-1em}



\SetKwProg{Fn}{function}{}{}
{
	\begin{algorithm}[tbh!]
		\DontPrintSemicolon
		\caption{Compute solution for a VLink and a datarate permutation}
		\label{alg:memoized}
		\Fn(){MDP($(\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4)$)}{

					\If{$F[(\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4)] \ne\phi$}
					{
						return $F[(\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4)]$
					}
					\If{$|(\mathcal{P}_{\bar{e}}^k, m_1)| = 1$}
					{
						%$p_1 \gets$ GetPath$(\mathcal{P}_{\bar{e}}^k, m_1)$\\
						%$d_1 \gets$ GetDatarate$(\mathcal{D}, m_4)$\\
						%Compute $n(\{p_1\},\{d_1\})$ using \eqn{eq:heu-eq4}\\
						Find $t$ that minimizes $n_t$ for $p_1 \in (\mathcal{P}_{\bar{e}}^k, m_1)$ and $d_1 \in (\mathcal{D}, m_4)$ using \eqn{eq:heu-eq4}\\
						\If{$t = \phi$}
						{$n \gets \infty$, $\mathcal{T} \gets \mathcal{S} \gets \phi$ \\}
						\Else{
						$\mathcal{S} \gets$ First-Fit($p_1, n_t$)\\
						\If{$\mathcal{S} = \phi$}
						{
							$n \gets \infty$, $\mathcal{T} \gets \mathcal{S} \gets \phi$ \\
						}
						\Else{
							$n \gets n_t$, $\mathcal{T} \gets \{t\}$ \\
						}
						}
						$F[(\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4)] \gets <n, \mathcal{T}, \mathcal{S}>$\\
                        return $<n, \mathcal{T}, \mathcal{S}>$
					}
					\Else
					{
						\ForEach{$i=1$ to $|(\mathcal{P}_{\bar{e}}^k, m_1)$}
						{
							$<n_i, \mathcal{T}_i, \mathcal{S}_i> \gets$ MDP($\{p_i\}, \{d_i\}$)
						}
						$n \gets \sum_{i=1}^{i=|(\mathcal{P}_{\bar{e}}^k, m_1)|} n_i$\\
						$\mathcal{T} \gets \bigcup_{i=1}^{i=|(\mathcal{P}_{\bar{e}}^k, m_1)|} \mathcal{T}_i$\\
						
						$\mathcal{S} \gets \bigcup_{i=1}^{i=|(\mathcal{P}_{\bar{e}}^k, m_1)|} \mathcal{S}_i$\\
						
						\If{$n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4)) = \infty$}
						{
							return $<\infty, \phi, \phi>$
						}
						\ElseIf{All paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$ are disjoint}
						{
							return $<n, \mathcal{T}, \mathcal{S}>$
						}
						\Else
						{
							$\zeta(\mathcal{P}_{\bar{e}}^k, m_1) \gets$ AllPerm$(\mathcal{P}_{\bar{e}}^k, m_1)$\\
							\ForEach{$(\mathcal{P}, m_1) \in \zeta(\mathcal{P}_{\bar{e}}^k, m_1)$}
							{
								Compute slice assignments in the order paths appear in $(\mathcal{P}, m_1)$ using First-Fit\\
							}
							Select the slice assignment that minimizes $frag((\mathcal{P}, m_1), (\mathcal{D}, m_4))$ using \eqn{eq:heu-eq6}\\
							Update $\mathcal{S}$ with the latest slice assignment\\
							return $<n, \mathcal{T}, \mathcal{S}>$
						}
						
					}

			}
		\end{algorithm}
		%\vspace{-0.5em}
}

All the aforementioned challenges have to be addressed jointly in order to find $\mathcal{A}_{\bar{e}}$.
As per \eqn{eq:heu-eq1}, to find $\mathcal{A}_{\bar{e}}$, we first explore all the possibilities of choosing the multi-set $(\mathcal{P}_{\bar{e}}^k, m_1)$. The number of multi-sets of cardinality $q$ on $k$ paths is termed as $k$ multichoose $q$ and is given by $\multiset{k}{q} = \binom{k+q-1}{q}$~\cite{pemmaraju2003computational}. Since the cardinality of $(\mathcal{P}_{\bar{e}}^k, m_1)$ can take any integer value from $1$ to $q$, we get $|\mathcal{M}{(\mathcal{P}_{\bar{e}}^k, m_1)}| = \displaystyle\sum_{i=1}^{i=q} \multiset{k}{i}$. Fortunately, the values of $k$ and $q$ in our problem is smaller than $10$ resulting in a reasonable number of multi-sets to enumerate. Now, for each of the path combinations $(\mathcal{P}_{\bar{e}}^k, m_1) \in \mathcal{M}{(\mathcal{P}_{\bar{e}}^k, m_1)}$, we have to find two multi-sets: one of tuples $(\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)}^{opt}, m_2)$ and another of slice indices $(S_{(\mathcal{P}_{\bar{e}}^k, m_1)}^{opt}, m_3)$ that minimize the number of spectrum slices for $(\mathcal{P}_{\bar{e}}^k, m_1)$, denoted as $n((\mathcal{P}_{\bar{e}}^k, m_1))$. Since the number of possible tuples and slice indices for $\bar{e}$ are $|\mathcal{T}_{\bar{e}}|$ and $|S|$, respectively, and cardinality of both $(\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_2)$ and $(\mathcal{S}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_3)$ have to be equal to that of $(\mathcal{P}_{\bar{e}}^k, m_1)$, the number of possibilities to explore for finding $(\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)}^{opt}, m_2)$ and $(\mathcal{S}_{(\mathcal{P}_{\bar{e}}^k, m_1)}^{opt}, m_3)$ are $\multiset{|\mathcal{T}_{\bar{e}}|}{|(\mathcal{P}_{\bar{e}}^k, m_1)|}$ and $\multiset{|\mathcal{S}|}{|(\mathcal{P}_{\bar{e}}^k, m_1)|}$, respectively.

\SetKwProg{Fn}{function}{}{}
{
	\begin{algorithm}[tbh!]
		\DontPrintSemicolon
		\caption{Compute solutions for a VLink}
		\label{alg:Compute-Backup}
		\Fn(){GetSolutions($G, \bar{e}, \mathcal{P}_{\bar{e}}^k, \mathcal{T}_{\bar{e}}$)}{
			$\mathcal{M}{(\mathcal{P}_{\bar{e}}^k, m_1)} \gets \phi$\\
		    \ForEach{$q=1$ to $N_q$}{
			$\mathcal{M}{(\mathcal{P}_{\bar{e}}^k, m_1)} \gets \mathcal{M}{(\mathcal{P}_{\bar{e}}^k, m_1)} \cup$ Multi-Set($\mathcal{P}_{\bar{e}}^k, q$)
			}
			\ForEach{$(\mathcal{P}_{\bar{e}}^k, m_1) \in \mathcal{M}{(\mathcal{P}_{\bar{e}}^k, m_1)}$}{
				{
					%$\mathcal{M}{(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)} \gets \phi$
					$\mathcal{M}{(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)} \gets$ Multi-Set($\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, |(\mathcal{P}_{\bar{e}}^k, m_1)|$)\\
					\ForEach{$(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4) \in \mathcal{M}{(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)}$}{
						$\zeta(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4) \gets$ AllPerm($(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$)
						\ForEach{$(\mathcal{D}, m_4) \in \zeta(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$}{
							$<n, \mathcal{T}, \mathcal{S}> \gets$ MDP($(\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4)$)
						}
						Find $\mathcal{T}^{best}$ and $\mathcal{S}^{best}$ that minimizes $n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4))$ using \eqn{eq:heu-eq3}
					}
					Find $(\mathcal{T}^{opt}, m_2)$ and $(\mathcal{S}^{opt}, m_3)$ that minimizes $n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4))$ using \eqn{eq:heu-eq2}\\
            $\mathcal{I}_{\bar{e}} \gets <(\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{T}^{opt}, m_2), (\mathcal{S}^{opt}, m_3)>$\\
            %$(\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)}^{opt}, m_2) \gets \mathcal{T}^{best}$\\
            %$(\mathcal{S}_{(\mathcal{P}_{\bar{e}}^k, m_1)}^{opt}, m_3) \gets \mathcal{S}^{best}$
			}
            Sort all $\mathcal{I}_{\bar{e}}$ in increasing order of $n(\mathcal{P}_{\bar{e}}^k, m_1)$ and return
		}
	}
		\end{algorithm}
		%\vspace{-0.5em}
}


%a solution is given by $\mathcal{J}_{\bar{e}(\mathcal{P}_{\bar{e}}^k, m_1)}=\{(\mathcal{T}_{\bar{e}(\mathcal{P}_{\bar{e}}^k, m_1)}, m_2), (S_{\bar{e}(\mathcal{P}_{\bar{e}}^k, m_1)}, m_3)\}$. Again, we can define an optimal solution for a given multi-set $(\mathcal{P}_{\bar{e}}^k, m_1)$ as follows:
%
%\vspace{-1.0em}
%\begin{equation}
%\mathcal{A}_{\bar{e}(\mathcal{P}_{\bar{e}}^k, m_1)} = \argminA_{\mathcal{J}_{\bar{e}(\mathcal{P}_{\bar{e}}^k, m_1)} \in \mathcal{M}{(\mathcal{T}_{\bar{e}(\mathcal{P}_{\bar{e}}^k, m_1)}, m_2)} \times \mathcal{M}{(\mathcal{S}_{\bar{e}(\mathcal{P}_{\bar{e}}^k, m_1)}, m_3)}}  n(\mathcal{J}_{\bar{e}(\mathcal{P}_{\bar{e}}^k, m_1)}) \label{eq:heu-eq2}
%\end{equation}
%\vspace{-1em}

To avoid dealing with such large number of possibilities, we take an alternate approach for computing both $(\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)}^{opt}, m_2)$ and $(S_{(\mathcal{P}_{\bar{e}}^k, m_1)}^{opt}, m_3)$. In this approach, we enumerate different multi-sets of datarates $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$ where $\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}$ is the set of all distinct datarates feasible for the paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$ and $m_4:\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)} \rightarrow N_q$ such that $|(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)| = |(\mathcal{P}_{\bar{e}}^k, m_1)| \wedge \displaystyle\sum_{d \in (\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)} d =  \bar{\beta}_{\bar{e}}$. For each $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$, we compute total spectrum requirement by assigning different datarates in $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$ to different paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$. We have to do this since to achieve a bandwidth (e.g., $600G$) using a path combination $\{p_1, p_2, p_3\} \in (\mathcal{P}_{\bar{e}}^k, m_1)$, not only different multi-sets of datarates (\eg $\{400, 100, 100\}$, $\{300, 200, 100\}$, and so on) but also different permutations of each of those multi-sets (\eg $\{400, 100, 100\}$, $\{100, 400, 100\}$, and so on) may require different number of slices. Hence, we explore all the permutations of the datarates of each of the multi-sets represented as $\zeta(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$ and find $(\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)}^{opt}, m_2)$ and $(S_{(\mathcal{P}_{\bar{e}}^k, m_1)}^{opt}, m_3)$ for the permutation that minimizes $n(\mathcal{P}_{\bar{e}}^k, m_1)$. More formally, if $\mathcal{M}{(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)}$ represents the set of all possible multi-sets of $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$ and $n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4))$ denotes the number of slices required to achieve the bandwidth $\bar{\beta}_{\bar{e}}$ using path and datarate combinations $(\mathcal{P}_{\bar{e}}^k, m_1)$ and $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$, respectively, we have

%if  represents the minimal number of slices required to achieve bandwidth $\bar{\beta}_{\bar{e}}$ on $(\mathcal{P}_{\bar{e}}^k, m_1)$ using $(\mathcal{D}, m_4)$,
%$n((\mathcal{P}_{\bar{e}}^k, m_1), \bar{\beta}_{\bar{e}}) = \min_{\forall (\mathcal{D}, m_4) \in (\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)!} n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4), \bar{\beta}_{\bar{e}})$.

\vspace{-1.0em}
\begin{equation}
n(\mathcal{P}_{\bar{e}}^k, m_1) = \displaystyle \min_{\forall \mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)} \in \mathcal{M}(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)} n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)) \label{eq:heu-eq2}
\end{equation}
\vspace{-1em}

Where, $n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4))$ can be computed by enumerating the slice requirement $n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4))$ for each permutation $(\mathcal{D}, m_4)$ of the datarate combination $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$ using $(\mathcal{P}_{\bar{e}}^k, m_1)$ as follows:

\vspace{-1.0em}
\begin{equation}
n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)) = \min_{\forall (\mathcal{D}, m_4) \in \zeta(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)}  n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4)) \label{eq:heu-eq3}
\end{equation}
\vspace{-1em}

%Among the different possible multi-sets of datarates, our objective is to find the datarate combination that minimizes the total number of spectrum.
The number of permutations of a multiset $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$ with $J$ distinct datarates is given by the multinomial coefficient as $\binom{|(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)|}{m(d_1), m(d_2),..., m(d_J)} = \frac{|(\mathcal{P}_{\bar{e}}^k, m_1)|!}{\Pi_{j=1}^J m(d_j)!}$, where $m(d_j)$ is the multiplicity of the $j$-th distinct datarate in $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$ \cite{brualdi1992introductory}. On other hand, number of possibilities for the multiset $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$ is $\multiset{|D|}{|(\mathcal{P}_{\bar{e}}^k, m_1)|}= \binom{|D|+|(\mathcal{P}_{\bar{e}}^k, m_1)|-1}{|(\mathcal{P}_{\bar{e}}^k, m_1)|}$, where $|D|$ is the number of distinct datarates in $\mathcal{R}$. Hence, we have to enumerate $\frac{(|D|+|(\mathcal{P}_{\bar{e}}^k, m_1)|-1)!}{(|D|-1)! \times \Pi_{j=1}^J m(d_j)!}$ possibilities to compute $n(\mathcal{P}_{\bar{e}}^k, m_1)$ using \eqn{eq:heu-eq2} and \eqn{eq:heu-eq3}. This reduces computational complexity as $|D|$ is much less than both $|\mathcal{T}_{\bar{e}}|$ and $|S|$.

%For a permutation $(\mathcal{D}, m_4) \in  \zeta(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$, we compute the total spectrum requirement $n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4))$ using the most spectrally efficient tuples feasible for each pair $(p_i, d_i)$, where $p_i$ is the $i$-th path in $(\mathcal{P}_{\bar{e}}^k, m_1)$ and $d_i$ is the $i$-th datarate in $(\mathcal{D}, m_4)$.

%$(\mathcal{T}_{(\mathcal{P}_{\bar{e}}^k, m_1)(\mathcal{D}, m_4)}, m_2)$ and $(S_{(\mathcal{P}_{\bar{e}}^k, m_1)(\mathcal{D}, m_4)}, m_3)$

Now, to optimally compute $n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4))$ for a datarate permutation $(\mathcal{D}, m_4) \in \zeta(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$, we adopt a Dynamic Programming (DP) approach. To apply DP, we have to divide the problem of computing $n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4))$ into sub-problems that have both overlapping sub-problems and optimal sub-structure properties. If $(\mathcal{D}, m_4) = \{d_1, d_2, .., d_{|(\mathcal{P}_{\bar{e}}^k, m_1)|}\}$, we divide the problem into $|(\mathcal{P}_{\bar{e}}^k, m_1)|$ sub-problems each of which is represented as $(\{p_i\}, \{d_i\})$, where $d_i$ is the $i$-th datarate in $(\mathcal{D}, m_4)$ and $p_i$ is the $i$-th path in $(\mathcal{P}_{\bar{e}}^k, m_1)$. Each $d_i \in (\mathcal{D}, m_4)$ such that $m(d_i)>1$ may result in multiple occurrences of the same sub-problems for paths $p_i \in (\mathcal{P}_{\bar{e}}^k, m_1)$ with $m(p_i)>1$. These sub-problems satisfy optimal sub-structure property as an optimal solution for $n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4))$ can be obtained by using optimal solutions to its sub-problems as follows:

\vspace{-1.0em}
\begin{equation}
n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4)) = \displaystyle\sum_{i=1}^{i=|(\mathcal{P}_{\bar{e}}^k, m_1)|} n(\{p_i\}, \{d_i\})
\label{eq:heu-eq5}
\end{equation}
\vspace{-1em}

For each sub-problem $(\{p_i\}, \{d_i\})$, also considered as the base cases in this problem, we use $\mathcal{R}$ to find the most spectrally efficient tuple $t$ with $d_i=t^{(d)}$ that has transmission reach of at least the length of the path $p_i$ and minimizes spectrum slice requirement for $(\{p_i\}, \{d_i\})$ as follows:

\vspace{-1.0em}
\begin{equation}
n(\{p_i\}, \{d_i\}) = \min_{\forall t \in \mathcal{T}_{{\bar{e}}p_i} | t^{(d)}=d_i \wedge r_t>=l(p_i)} n_t
\label{eq:heu-eq4}
\end{equation}
\vspace{-1em}

We can then pick $n(\{p_i\}, \{d_i\})$ slices along the path $p_i$ using any good slice assignment approach (\eg first fit \cite{chatterjee2015routing}). In addition to $n(\{p_i\}, \{d_i\})$, the sub-problem $(\{p_i\}, \{d_i\})$ also returns a tuple $t$ and a slice selection of contiguous and free $n_t$ slices along the path $p_i$. However, it may be possible that the substrate links present in $p_i$ do not have $n_t$ contiguous slices, turning the sub-problem into an infeasible one. We handle such cases by setting $n(\{p_i\}, \{d_i\})$ to a very large value (\eg $\infty$) and returning null for tuple and slice selection. We also observe that many sub-problems are repeated across different permutations of a datarate multi-set, different multi-sets of datarates, and even different path combinations in the whole solution space allowing us to use memoization for the already computed solutions of the sub-problems.

%By merging the results of these sub-problems, we can compute $n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4))$ as follows:

Although we can combine the tuples returned by the sub-problems to get a valid tuple selection for the combinations $(\mathcal{P}_{\bar{e}}^k, m_1)$ and $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4))$, we cannot do the same for slice indices. The reasons are twofold. First, spectrum resources are shared among the paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$ that have common substrate links. Second, sub-problems are solved independently without considering the shared spectrum resources on common substrate links. As a result, slice selections to two sub-problems involving two paths such as $(\{p_1\}, \{100\})$ and $(\{p_2\}, \{200\})$ with a common substrate link can use a common spectrum slice. However, these slice selections may become invalid when merging the solutions for $(\{p_1\}, \{100\})$ and $(\{p_1\}, \{200\})$ to get the slice selection for $(\{p_1, p_1\},\{100, 200\})$ due to violation of spectrum non-overlapping requirement. The same is true for the solutions to the sub-problems involving the same paths such as $(\{p_1\}, \{100\})$ and $(\{p_1\}, \{200\})$. However, the slice assignments for the sub-problems can be readily used in the combine step for the paths that are disjoint.

%Otherwise, we check whether the slice selections of the sub-problems have any overlap. If there is no overlap, we are good at using the solutions of the sub-problems. The critical case is the one that has overlaps in spectrum slices.

We take these cases into account to combine the solutions of the sub-problems. First, if all the paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$ are disjoint we do nothing but using the spectrum selections from the sub-problems. Otherwise, we scrap the slice selections of the sub-problems and find a new slice selection using the tuples returned by the sub-problems. To do so, we have to select $n(\{p_i\}, \{t_i^{(d)}\})$ contiguous and un-occupied slices along each path $p_i \in (\mathcal{P}_{\bar{e}}^k, m_1)$. The order in which we assign slices to these paths has an impact on the corresponding slice selection. For instance, slice selections to $|(\mathcal{P}_{\bar{e}}^k, m_1)|-1$ paths may create fragmentation to one of the paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$ in such a way that the path does not have the required number of contiguous and un-occupied slices for the last slice assignment. Therefore, we enumerate all the permutations of the paths represented as $\zeta(\mathcal{P}_{\bar{e}}^k, m_1)$ to find all the feasible slice selections. For a given permutation $(\mathcal{P}, m_1) \in \zeta(\mathcal{P}_{\bar{e}}^k, m_1)$ assign slices to paths in the order a path appears in a permutation. This will require to explore $\frac{|(\mathcal{P}_{\bar{e}}^k, m_1)|!}{\Pi_{j=1}^{J_{(\mathcal{P}_{\bar{e}}^k, m_1)}} m(p_j)!}$ possibilities where $J_{(\mathcal{P}_{\bar{e}}^k, m_1)}$ is the total number of distinct paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$ and $p_j$ is the j-th distinct path in $(\mathcal{P}_{\bar{e}}^k, m_1)$.

%We take these cases into account to combine the solutions of the sub-problems. First, if all the paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$ are disjoint we do nothing but using the spectrum selections from the sub-problems. Otherwise, we scrap the slice selections of the sub-problems and find a new slice selection using the tuples returned by the sub-problems. To do so, we have to select $n(\{p_i\}, \{t_i^{(d)}\})$ contiguous and un-occupied slices for the $<$path, tuple$>$=($p_i$, $t_i$) pair, and there are $|(\mathcal{P}_{\bar{e}}^k, m_1)|$ number of such pairs. The order in which we assign slices to those pairs has an impact on the corresponding slice selection. For instance, slice selections to $|(\mathcal{P}_{\bar{e}}^k, m_1)|-1$ $<$path, tuple$>$ pairs may create fragmentation to one of the paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$ in such a way that the path does not have the required number of contiguous and un-occupied slices for last $<$path, tuple$>$ pair. Therefore, we have to explore all possible orders of $<$path, tuple$>$ pairs to find all the feasible slice selections. To do so, we enumerate all the permutations of the paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$ and construct $<$path, tuple$>$ pairs by combining a path $p_i$ and the corresponding tuple $t_i$ returned by its sub-problem. This will require to explore $\frac{|(\mathcal{P}_{\bar{e}}^k, m_1)|!}{\Pi_{j=1}^{J_{(\mathcal{P}_{\bar{e}}^k, m_1)}} m(p_j)!}$ possibilities where $J_{(\mathcal{P}_{\bar{e}}^k, m_1)}$ is the total number of distinct paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$ and $p_j$ is the j-th distinct path in $(\mathcal{P}_{\bar{e}}^k, m_1)$.

Note that all the path permutations with a feasible slice selection have the same value for $n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4))$ as slice selection does not change the number of spectrum slice requirement. However, it is possible that we do not find any feasible slice selection even by exploring all possible permutations of $\zeta(\mathcal{P}_{\bar{e}}^k, m_1)$. In such a case, we make the solution invalid by setting $n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4)) = \infty$. In addition, to decrease the blocking probability of later VLinks without sacrificing the optimality of the current solution, we choose the permutation $(\mathcal{P}, m_1) \in \zeta(\mathcal{P}_{\bar{e}}^k, m_1)$ that has a feasible slice selection and minimizes spectrum fragmentation $frag((\mathcal{P}, m_1), (\mathcal{D}, m_4))$ on the paths in the remaining VLinks of a VN. If $\bar{E}_{r} \subset \bar{E}$ is the set of remaining VLinks when we find solution for $\bar{e}$, we can define defined as follows:

\vspace{-1.0em}
\begin{equation}
frag((\mathcal{P}, m_1), (\mathcal{D}, m_4)) = \sum_{\bar{e}_{r} \in \bar{E}_{r}} \sum_{\forall p \in (\mathcal{P}_{\bar{e}_{r}}^k, m_1)} \frac{\text{free slice count in} \bar{e}_{r}}{\text{non-contiguous block count in} \bar{e}_{rem}}
\label{eq:heu-eq6}
\end{equation}
\vspace{-1em}




%in the permutation returned by different sub-problems of computing $n((\mathcal{P}_{\bar{e}}^k, m_1), (\mathcal{D}, m_4))$

%and choose the spectrum slice selection for the permutation that minimizes spectrum fragmentation on the paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$.

%Note that all permutations of paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$ with a valid slice selection require the same number of spectrum slices

\subsection{Heuristic solution for a VN}\label{sec:vn-heuristic}
In addition, for a VN with multiple VLinks, there are combinatorial number of permutations in which the solutions for the VLinks can be computed. Therefore, a heuristic algorithm should take into account all these aspects to find a feasible solution for a VN in a reasonable time. We now discuss how we address these challenges in our heuristic algorithm.

%^spectrum slice selection needs extra care when the paths in $(\mathcal{P}_{\bar{e}}^k, m_1)$ that have common substrate links. Hence, slice selections to two sub-problems such as $(\{p_1\}, \{100\})$ and $(\{p_1\}, \{200\})$ may become invalid when merging them to get slice selection for $(\{p_1, p_1\},\{100, 200\})$ due to spectrum non-overlapping constraints. Similarly, even though there are valid slice assignments to two sub-problems such as $(\{p_1\}, \{100\})$ and $(\{p_2\}, \{200\})$ where $p_1$ and $p_2$ have at least one common substrate link, there may be no feasible slice assignments for $(\{p_1, p_2\},\{100, 200\})$ due to spectrum non-overlapping and capacity constraints. We take into account these cases by setting the corresponding number of slice requirement values $\infty$ turning the original problem an infeasible one.

%Therefore, in the conquer step, we retrieve the selected tuples of all the sub-problems of a permutation and assign spectrum slices while satisfying spectrum contiguity, capacity, and non-overlapping use of spectrum slice constraint.

%In this approach, we divide the problem of finding $(\mathcal{T}_{\bar{e}(\mathcal{P}_{\bar{e}}^k, m_1)}, m_2)$ to achieve $\bar{\beta}_{\bar{e}}$ into $|(\mathcal{P}_{\bar{e}}^k, m_1)|$ sub-problems each of which finds a tuple to achieve a datarate $d \le \bar{\beta}_{\bar{e}}$ along each path present in $(\mathcal{P}_{\bar{e}}^k, m_1)$.

%The reason for exploring all the permutations of a multi-set $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4) = \{400, 100, 100\}$ for the path combination $\{p_1, p_2, p_3\}$ is that different permutations such as $\{400, 100, 100\}$ and $\{100, 400, 100\}$ may require different number of spectrum slices for $\{p_1, p_2, p_3\}$.


% we first find all the multi-sets of data rates $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$ where $m_4:\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)} \rightarrow N_q$ such that $|(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)| = |(\mathcal{P}_{\bar{e}}^k, m_1)| \wedge \displaystyle\sum_{d \in (\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)} d =  \bar{\beta}_{\bar{e}}$ and find the permutation that minimizes the total number of spectrum slices.

%In this approach, we explore all the permutations of the elements of all the multi-sets of data rates $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$ where $m_4:\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)} \rightarrow N_q$ such that $|(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)| = |(\mathcal{P}_{\bar{e}}^k, m_1)| \wedge \displaystyle\sum_{d \in (\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)} d =  \bar{\beta}_{\bar{e}}$ and find the permutation that minimizes the total number of spectrum slices.



%to achieve the datarates present in a permutation of $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$ divide the problem into sub-problems consisting of the elements present in one permutations of the datarates of $(\mathcal{D}_{(\mathcal{P}_{\bar{e}}^k, m_1)}, m_4)$








==> ilp-formulation-report.tex <==
\section{Problem Formulation}\label{sec:ilp}
We present a path-based ILP formulation for the VNE over EON problem, \ie we provide the set of possible paths that can be used to embed VLinks as in input to the formulation.
%We first provide a Quadratic Integer Program (QIP) formulation for the joint spare capacity allocation and survivable embedding problem in \sect{subsec:qip}, followed by a discussion on the complexity of the QIP in \sect{subsec:hardness}. We then describe the transformation of the QIP to an ILP in \sect{subsec:ilp}.

%We now present the notations:\newline
%We first present our decision variables (\sect{subsec:c_dvariables}). Then we introduce the constraints (\sect{subsec:c_constraints}) followed by the objective function of our formulation ((\sect{subsec:c_objective}).
%\begin{tabular}{ l p{2.75 in} }
%$\mathcal{P}_{\bar{e}}^k:$ & set of candidate paths for the VLink $\bar{e} \in \bar{E}$\\
%$\mathcal{T}_{\bar{e}p}:$ &  set of admissible tuples for the VLink $\bar{e}$ on the path $p \in \mathcal{P}_{\bar{e}}^k$\\
%$n_{t}:$ & the number of required frequency slices for the tuple $t \in T$\\
%$q:$ & the maximum number of splits a VLink can have\\
%$\delta_{pe}:$ &  1 if $e \in E$ is on the path $p \in \mathcal{P}$, 0 otherwise\\
%$src(p):$ & Source substrate node of the path p\\
%$dest(p):$ & Destination substrate node of the path p\\
%$src(\bar{e}):$ & Source virtual node of the link $\bar{e} \in \bar{E}$ \\
%$dest(\bar{e}):$ & Destination virtual node of the link $\bar{e} \in \bar{E}$\\
%\end{tabular}
%\section{ILP Formulation for minimizing spectrum usage}\label{subsec:main_ilp}
\subsection{Decision Variables}\label{subsec:c_dvariables}
A VNode is mapped to exactly one SNode from its location constraint set, denoted by the following decision variable:%\vspace{-0.25em}
\begin{align*}
x_{\bar{u}u} = \begin{cases}
1 & \text{if } \bar{u} \in \bar{V} \text{ is mapped to } u \in V\\
0 & \text{otherwise}
\end{cases}
\end{align*}
We allow VLink splitting for embedding, \ie satisfy the demand of a VLink by provisioning slices over multiple SPaths up to a maximum of $q$ SPaths as $q$ is the maximum number of allowable splits. Slice provisioning over multiple SPaths can be done using a combination of the following two cases: (i) allocate contiguous sets of slices on distinct SPaths; (ii) allocate different contiguous sets of slices on the same SPath (with identical or different transmission configuration). The latter represents a scenario when there are sufficient slices available over an SPath, however, the SPath length does not allow provisioning the total required data-rate using a single contiguous set of slices. To represent the second case, we assume each transmission configuration for an SPath can be instantiated multiple times (up to a maximum of $q$ times as total number of splits cannot exceed $q$ regardless of the case). The following variable relates a VLink to an SPath and an instance of a transmission configuration on that SPath:%\vspace{-0.25em}
\begin{align*}
w_{\bar{e}pti} = \begin{cases}
1 & \text{if } \bar{e} \in \bar{E} \text{ uses } i\text{-th} \text{ instance of } t \in \mathcal{T}_{\bar{e}p}\\
  & \text{ on path } p \in \mathcal{P}_{\bar{e}}^k\\
0 & \text{otherwise}
\end{cases}
\end{align*}


Finally, the following decision variable creates the relationship between a mapped SPath and the slices in its SLinks:%{-0.25em}


\begin{align*}
y_{\bar{e}ptis} = \begin{cases}
1 & \text{if } \bar{e} \in \bar{E} \text{ uses slice } s \in S \text{ on path } p \in \mathcal{P}_{\bar{e}}^k\\
  & \text{with the } i\text{-th} \text{ instance of } t \in \mathcal{T}_{\bar{e}p}\\
0 & \text{otherwise}
\end{cases}
\end{align*}
\vspace{0em}
%\begin{tabular}{ l p{2.75 in} }

%$w_{\bar{e}pti}:$ & 1, if $\bar{e} \in \bar{E}$ uses $i_{th}$ instance of tuple $t \in \mathcal{T}_{\bar{e}p}$ on path $p \in \mathcal{P}_{\bar{e}}^k$, 0 otherwise \\
%$y_{\bar{e}ptis}:$ & 1, if $\bar{e} \in \bar{E}$ uses slice $s \in S$ on path $p \in \mathcal{P}_{\bar{e}}^k$ with $i_{th}$ instance of tuple $t \in \mathcal{T}_{\bar{e}p}$, 0 otherwise \\
%\end{tabular}

%\begin{comment}
%The VNode to SNode mapping is denoted using the following decision variable:
%\vspace{-0.5em}
%\begin{align*}
%x_{\bar{u}u} & =\left\{ \begin{array}{rl}
%1 & \text{if } \bar{u} \in \bar{V} \text{ is mapped to } u \in V,\\
%0 & \text{otherwise}.
%\end{array}\right.
%\end{align*}
%\vspace{-1.25em}
%
%The following decision variable indicates the mapping between a VLink $(\bar{u}, \bar{v}) \in \bar{E}$ and a path $p \in \mathcal{P}_{\bar{e}}^k$ and an instance of a tuple $t \in \mathcal{T}_{\bar{e}p}$ :
%\vspace{-0.5em}
%\begin{align*}
%w_{\bar{e}pti} & =\left\{ \begin{array}{rl}
%1 & \text{if } \bar{e} \in \bar{E} \text{ uses } i_{th} \text{ instance of tuple } t \in \mathcal{T}_{\bar{e}p} \text{ on path } p \in \mathcal{P}_{\bar{e}}^k,\\
%0 & \text{otherwise}.
%\end{array}\right.
%\end{align*}
%\vspace{-1em}
%
%The following decision variable indicates the assignment of spectrum slices to a VLink $(\bar{u}, \bar{v}) \in \bar{E}$ that uses path $p \in \mathcal{P}_{\bar{e}}^k$ and an instance of a tuple $t \in \mathcal{T}_{\bar{e}p}$ :
%\vspace{-0.5em}
%\begin{align*}
%y_{\bar{e}ptis} & =\left\{ \begin{array}{rl}
%1 & \text{if } \bar{e} \in \bar{E} \text{ uses slice } s \in S \text{ on path } p \in \mathcal{P}_{\bar{e}}^k \text{ with } i_{th} \text{ instance of tuple } t \in \mathcal{T}_{\bar{e}p},\\
%0 & \text{otherwise}.
%\end{array}\right.
%\end{align*}
%\vspace{-1em}
%\end{comment}

%\begin{align*}
%y_{\bar{e}ptis} & =\left\{ \begin{array}{rl}
%1 & \text{if } \bar{e} \in \bar{E} \text{ uses slice } s \in S \text{ on path } p \in \mathcal{P}_{\bar{e}}^k \text{ with } i_{th} \text{ instance of tuple } t \in \mathcal{T}_{\bar{e}p},\\
%0 & \text{otherwise}.
%\end{array}\right.
%\end{align*}




\subsection{Constraints}\label{subsec:c_constraints}
\paragraph{VNode Mapping Constraints}
We ensure by \eqn{eq:nmap1} and \eqn{eq:nmap2} that each VNode is mapped to an SNode satisfying the location constraints. Then, \eqn{eq:nmap3} constraints an SNode to host at most one VNode from the same VN. Note that VNode mapping follows from VLink mapping, since there is no cost associated with the VNode mapping.
%Provisioning of a VNode should be done according to the location constraint as provided in the input.
%\begin{align}
%\forall \bar{u} \in \bar{V}: \displaystyle\sum_{u \in N} y_{\bar{u}u} = 1
%\end{align}
%A VNode should be provisioned at exactly one node in the substrate network. Also, a SNode will not host more than one VNode from the same virtual network request. Finally, a VNode is mapped to exactly one SNode. We ensure these by the following constraints:


\vspace{-0em}
\begin{align}
\forall \bar{u} \in \bar{V},\forall u \in V: x_{\bar{u}u} \leq c_{\bar{u}u}\label{eq:nmap1}\\
\forall \bar{u} \in \bar{V}: \displaystyle\sum_{{u} \in {V}} x_{\bar{u}u} = 1\label{eq:nmap2}\\
\forall u \in V: \displaystyle\sum_{\bar{u} \in \bar{V}} x_{\bar{u}u} \leq 1\label{eq:nmap3}
\end{align}
%\vspace{-1em}

\paragraph{VLink demand constraints}
We provision a VLink by splitting it across multiple (up to $q$) SPaths. Constraint \eqn{eq:demand} ensures that for each VLink $\bar{e} \in \bar{E}$, the sum of data-rates resulting from applying the selected transmission configuration on the selected splits is equal or larger than the VLink's demand. Then, \eqn{eq:max-split} enforces an upper limit on the number of splits.
%  enforces the maximum number (\ie q) of splits for each link mapping.


%\vspace{-0.8em}
%\begin{align}
%\forall \bar{e} \in \bar{E}: \displaystyle\sum_{\forall p \in \mathcal{P}_{\bar{e}}^k} \sum_{\forall t \in \mathcal{T}_{\bar{e}p}} \sum_{i = 1}^{q} (w_{\bar{e}pti}\times t^{(d)}) & = \bar{\beta}_{\bar{e}} \label{eq:demand}
%\end{align}

\begin{align}
\forall \bar{e} \in \bar{E}: \bar{\beta}_{\bar{e}} \leq \displaystyle\sum_{\forall p \in \mathcal{P}_{\bar{e}}^k} \sum_{\forall t \in \mathcal{T}_{\bar{e}p}} \sum_{i = 1}^{q} (w_{\bar{e}pti}\times t^{(d)}) \label{eq:demand}
\end{align}


%\vspace{-0.8em}
\begin{align}
\forall \bar{e} \in \bar{E}: \displaystyle\sum_{\forall p \in \mathcal{P}_{\bar{e}}^k} \sum_{\forall t \in \mathcal{T}_{\bar{e}p}} \sum_{i = 1}^{q} w_{\bar{e}pti} & \leq q \label{eq:max-split}
\end{align}

%\vspace{-0.8em}
%\begin{equation}
%\begin{split}
%\forall \bar{e} \in \bar{E}, \forall p \in \mathcal{P}_{\bar{e}}^k, \forall t \in \mathcal{T}_{\bar{e}p}, 1 \leq i \leq q:\\ \displaystyle\sum_{\forall s \in S} y_{\bar{e}ptis} = n(\zeta(p, t), t) \times w_{\bar{e}pti} \end{split}\label{eq:sl-demand}
%\end{equation}
\paragraph{Slice assignment and Spectral Contiguity constraints}
We ensure by \eqn{eq:sl-demand} that if a path $p$ is selected with a specific transmission configuration $t$, then the required number of slices $n_t$ to support the data-rate $t^{(d)}$ is allocated on the path. \eqn{eq:sl-once} ensures that each slice on an SLink is allocated to at most one path. Finally, we ensure the slices allocated on each link of a path are contiguous, \ie consecutive slices are adjacent to each other in the frequency spectrum by \eqn{eq:contiguity}.
\begin{align}
\forall \bar{e} \in \bar{E}, \forall p \in \mathcal{P}_{\bar{e}}^k, \forall t \in \mathcal{T}_{\bar{e}p}, 1 \leq i \leq q: \nonumber \\ \displaystyle\sum_{\forall s \in S} y_{\bar{e}ptis} = n_t \times w_{\bar{e}pti}\label{eq:sl-demand}
\end{align}\vspace{-0em}


\begin{align}
\forall e \in E, \forall s \in S:\nonumber\\ \displaystyle\sum_{\forall \bar{e} \in \bar{E}} \sum_{\forall p \in \mathcal{P}_{\bar{e}}^k} \sum_{\forall t \in \mathcal{T}_{\bar{e}p}} \sum_{i = 1}^{q} w_{\bar{e}pti} \times y_{\bar{e}ptis} \times \delta_{pe}  \leq 1 \label{eq:sl-once}
\end{align}

\vspace{-0em}
%\vspace{-1.0em}
\begin{equation}
\begin{split}
\forall \bar{e} \in \bar{E}, \forall p \in \mathcal{P}_{\bar{e}}^k, \forall t \in \mathcal{T}_{\bar{e}p}, 1 \leq i \leq q, 1 \leq s \leq |S| - 1:\\ \displaystyle \sum_{s' = s+2}^{|S|} y_{\bar{e}ptis'} \leq |S| \times (1-y_{\bar{e}ptis}+ y_{\bar{e}pti(s+1)}) \end{split}\label{eq:contiguity}
\end{equation}
%\vspace{-1em}


%For reliability problem
\paragraph{Reliability constraints}
\eqn{eq:rel} ensures that for each single substrate link failure scenario, the aggregate data rate of the unaffected splits of a VLink $\bar{e} \in \bar{E}$ is at least $BSR_{\bar{e}}$ fraction of the original VLink demand.
\begin{align}
\forall \bar{e} \in \bar{E}, \forall e \in E: (\displaystyle \sum_{\forall p \in \mathcal{P}_{\bar{e}}^k} \sum_{\forall t \in \mathcal{T}_{\bar{e}p}} \sum_{i = 1}^{q} w_{\bar{e}pti} \times t^{(d)}) - (\sum_{\forall p \in \mathcal{P}_{\bar{e}}^k} \sum_{\forall t \in \mathcal{T}_{\bar{e}p}} \sum_{i = 1}^{q} w_{\bar{e}pti} \times t^{(d)} \times \delta_{pe})  \geq BSR_{\bar{e}} \times \bar{\beta}_{\bar{e}} \label{eq:rel}
\end{align}



\begin{comment}
\paragraph{Latency Constraints}
Recall from \sect{subsec:vn_lat} that the VN embedding has to satisfy a set of latency constraints $\mathcal{L}(\bar{G})$. Since each latency constraint $\ell \in \mathcal{L}(\bar{G})$ involves some VLinks, we first convert \eqn{eq:vlink-lat} to a linear constraint to find the latency of each VLink from its set of embedding paths as follows:
%find the latency of a VLink by computing the maximum latency of each VLink defined by \eqn{eq:vlink-lat} as follows:
\begin{align}
\forall \bar{e} \in \bar{E}, \forall p \in \mathcal{P}_{\bar{e}}^k, \forall t \in \mathcal{T}_{\bar{e}p}, 1 \leq i \leq q: w_{\bar{e}pti} \times L_{p} \leq vlink\_lat_{\bar{e}} \label{eq:diff1}
\end{align}

The following constraint uses \eqn{eq:diff1} to ensure that each latency constraint $\ell \in \mathcal{L}(\bar{G})$ is satisfied:
\begin{align}
\forall \ell \in \mathcal{L}(\bar{G}): \sum_{\forall \bar{e} \in \ell^{(\bar{a})}} vlink\_lat_{\bar{e}}  \leq \ell^{(L)}\label{eq:lat}
\end{align}


\paragraph{Differential Delay Constraints}
As discussed in \sect{subsec:diff_delay}, the embedding of each VLink has to satisfy the differential delay requirement represented by \eqn{eq:l-dd}. We use \eqn{eq:diff1} and \eqn{eq:diff2} to find the maximum and minimum delay of each VLink, respectively. In \eqn{eq:diff2}, extra care is needed to avoid getting zero as the minimum delay of a VLink induced by a non-selected path, tuple, and instance combination. The second term in the right hand size of \eqn{eq:diff2} allows to avoid such cases assuming that $\lambda$ is sufficiently larger than the maximum value of $L_p$ in the EON. For a non-selected path combination, second term on the right hand side of \eqn{eq:diff2} becomes dominant, generating the constraint $min\_delay(\bar{e}) \leq \lambda$. For a selected path, tuple, and instance combination, the second term becomes zero and the first term generates the constraint $min\_delay(\bar{e}) \leq L_{p}$. As $\lambda >> L_p$, $min\_delay(\bar{e}) \leq L_{p}$ dominates over $min\_delay(\bar{e}) \leq \lambda$ to generate the minimum delay of a VLink as the minimum delay of all the selected path, tuple, and instance combinations. Finally, \eqn{eq:diff3} uses \eqn{eq:diff1} and \eqn{eq:diff2} to enforce the differential delay requirement for each VLink:

\begin{align}
\forall \bar{e} \in \bar{E}, \forall p \in \mathcal{P}_{\bar{e}}^k, \forall t \in \mathcal{T}_{\bar{e}p}, 1 \leq i \leq q: min\_delay(\bar{e}) \leq w_{\bar{e}pti} \times L_{p} + (1-w_{\bar{e}pti})\times \lambda \label{eq:diff2}\\
\forall \bar{e} \in \bar{E}: vlink\_lat_{\bar{e}} - min\_delay(\bar{e}) \leq DD_{max}\label{eq:diff3}
\end{align}
\end{comment}

\paragraph{Coordination between node and link mapping}
\eqn{eq:coord} ensures that two endpoints of a VLink $\bar{e} \in \bar{E}$ are mapped to the source and destination substrate nodes of an SPath $p$ only when $p$ is used for embedding $\bar{e}$.


\begin{equation}\begin{split}
\forall \bar{e} \in \bar{E}, \forall p \in \mathcal{P}_{\bar{e}}^k, \forall t \in \mathcal{T}_{\bar{e}p}, 1 \leq i \leq q: \\ x_{src(\bar{e})src(p)} \times x_{dst(\bar{e})dst(p)} \geq w_{\bar{e}pti} \end{split}\label{eq:coord}
\end{equation}

\eqn{eq:coord} is a non-linear constraint. To linearize it, we introduce a new binary variable $z_{\bar{e}pti}$ defined as:

\begin{align*}
	z_{\bar{e}pti} = \begin{cases}
		1 & \text{if } x_{src(\bar{e})src(p)} \times x_{dst(\bar{e})dst(p)} = 1\\
		0 & \text{otherwise}
	\end{cases}
\end{align*}

We can enforce the definition of $z_{\bar{e}pti}$ using the following constraints:

\begin{equation}
		\forall \bar{e} \in \bar{E}, \forall p \in \mathcal{P}_{\bar{e}}^k, \forall t \in \mathcal{T}_{\bar{e}p}, 1 \leq i \leq q: \\ z_{\bar{e}pti} \le x_{src(\bar{e})src(p)}\label{eq:lin1}
\end{equation}

\begin{equation}
\forall \bar{e} \in \bar{E}, \forall p \in \mathcal{P}_{\bar{e}}^k, \forall t \in \mathcal{T}_{\bar{e}p}, 1 \leq i \leq q: \\ z_{\bar{e}pti} \le x_{dst(\bar{e})dst(p)}\label{eq:lin2}
\end{equation}
	
\begin{equation}
\forall \bar{e} \in \bar{E}, \forall p \in \mathcal{P}_{\bar{e}}^k, \forall t \in \mathcal{T}_{\bar{e}p}, 1 \leq i \leq q: \\ z_{\bar{e}pti} \ge x_{src(\bar{e})src(p)} + x_{dst(\bar{e})dst(p)}\label{eq:lin3} - 1
\end{equation}

Using the variable $z_{\bar{e}pti}$, we can linearize \eqn{eq:coord} as follows:
\begin{equation}
\forall \bar{e} \in \bar{E}, \forall p \in \mathcal{P}_{\bar{e}}^k, \forall t \in \mathcal{T}_{\bar{e}p}, 1 \leq i \leq q: \\ z_{\bar{e}pti} \geq w_{\bar{e}pti} \label{eq:lin4}
\end{equation}



%using a technique similar to~\cite{lin2017virtual} as follows:

\subsection{Objective Function}\label{subsec:c_objective}
Our cost function minimizes the total number of spectrum slices required to embed all the VLinks as shown in the first part of \eqn{obj}. However, to break ties among multiple solutions with the same total number of slices, we use the second term in \eqn{obj} that prefers the solution with the minimum number of splits. This gives us the following objective function:
% For a single VLink $(\bar{u},\bar{v}) \in \bar{E}$, the cost of embedding on a substrate network is:
%\begin{align*}
%\displaystyle\sum_{\forall(u,v) \in E} x_{uv}^{\bar{u}\bar{v}} \times C_{uv} \times (b_{\bar{u}\bar{v}} + S_{\bar{u}\bar{v}})
%\end{align*}
%We minimize the cost of embedding all the VLinks on the substrate network. Therefore, we have the following objective function:
%\vspace{-0.25em}


\begin{equation}
\begin{split}
\text{minimize} (\displaystyle\sum_{\forall \bar{e} \in \bar{E}} \sum_{\forall p \in \mathcal{P}_{\bar{e}}^k} \sum_{\forall t \in \mathcal{T}_{\bar{e}p}} \sum_{i=1}^{q} \sum_{\forall s \in S} y_{\bar{e}ptis} + \\ \epsilon_1 \times \sum_{\forall \bar{e} \in \bar{E}} \sum_{\forall p \in \mathcal{P}_{\bar{e}}^k} \sum_{\forall t \in \mathcal{T}_{\bar{e}p}} \sum_{i=1}^{q} w_{\bar{e}pti})\end{split}
\label{obj}
\end{equation}
$\epsilon_1$ is chosen in a way that the second term is effective only when multiple solutions have same value for the first part.

%Our cost function minimizes the total number of spectrum slices required to embed all the VLinks as shown in \eqn{obj}. As opposed to previous phases, we do not use any tie-breaker in the objective function as this increases the computational complexity of the ILP formulation, thus reducing its scalability. In previous phases, we have already observed that there might be multiple optimal solutions that have the same value for the objective function \eqn{obj} despite using different number of splits up to a maximum of $q$ splits, paths with different lengths, and so on. The ILP formulation with the objective function \eqn{obj} will return the first optimal solution it encounters. However, adding tie breaker components to \eqn{obj} can discriminate among those solutions at the cost of increased complexity.
% to break tie the among
%The intuition behind using this tie-breaker function is that carrying the same number of spectrum slices over a shorter distance path incurs lower cost than carrying the same number of slices over a longer distance path due to lower energy consumption and other operational expenses. However, we have observed that there can be multiple solutions with the same value for both the primary and secondary objective functions. To break ties among these solutions, we use the third term in \eqn{obj} that minimizes the total number of splits used by all the VLinks. This gives us the following objective function:

% For a single VLink $(\bar{u},\bar{v}) \in \bar{E}$, the cost of embedding on a substrate network is:
%\begin{align*}
%\displaystyle\sum_{\forall(u,v) \in E} x_{uv}^{\bar{u}\bar{v}} \times C_{uv} \times (b_{\bar{u}\bar{v}} + S_{\bar{u}\bar{v}})
%\end{align*}
%We minimize the cost of embedding all the VLinks on the substrate network. Therefore, we have the following objective function:
%\vspace{-0.25em}


%\begin{equation}
%\begin{split}
%\text{minimize} \left ( \displaystyle\sum_{\forall \bar{e} \in \bar{E}} \sum_{\forall p \in \mathcal{P}_{\bar{e}}^k} \sum_{\forall t \in \mathcal{T}_{\bar{e}p}} \sum_{i=1}^{q} \sum_{\forall s \in S} y_{\bar{e}ptis} \times |p| \right ) \end{split}
%\label{obj}
%\end{equation}
%The weights $\epsilon_1$ and $\epsilon_2$ in \eqn{obj} are chosen in a way that the second term is effective only when multiple optimal solutions have same value for the first part and the third term is only effective when there are multiple solutions with the same values for both the first and second objectives.

% some of the
\begin{comment}
\section{Problem Variant with Load-balancing Objective}\label{subsec:variation}
One drawback of using the objective function \eqn{obj} is that it may overuse spectrum slices on SLinks that appear more often on the shortest SPaths than other SLinks, in this way leaving insufficient number of contiguous slices on those SLinks to be used by the later VN requests. One strategy to avoid creating such bottleneck SLinks is to use an objective function that can balance spectrum usage across the SLinks.  One way of mathematically modeling such load-balancing is to use the objective function of minimizing the maximum index of allocated slice across all the SLinks in the SN \cite{wang2011study}. However, this load-balancing strategy may potentially select a longer SPath in order to minimize the maximum slice index, thus increasing the total spectrum usage. To achieve the objective of load-balancing instead of minimizing the total slice usage, we need to augment constraints \eqn{eq:var1} to our ILP formulation presented earlier and replace the objective function \eqn{obj} with \eqn{obj-1}.
\begin{equation}
\begin{split}
\forall e \in E, \forall \bar{e} \in \bar{E}, \forall p \in \mathcal{P}_{\bar{e}}^k, \forall t \in \mathcal{T}_{\bar{e}p}, 1 \leq i \leq q, \forall s \in S: s \times y_{\bar{e}ptis} \le Max\_Slice\_Index
\end{split}\label{eq:var1}
\end{equation}

% that minimizes the maximum index of
%\begin{equation}
%\begin{split}
%	\forall e \in E: Used\_Slice\_Index(e) \le Max\_Slice\_Index
%\end{split}\label{eq:var2}
%\end{equation}

\begin{equation}
\begin{split}
\text{minimize} (Max\_Slice\_Index + \epsilon_2 \times \displaystyle\sum_{\forall \bar{e} \in \bar{E}} \sum_{\forall p \in \mathcal{P}_{\bar{e}}^k} \sum_{\forall t \in \mathcal{T}_{\bar{e}p}} \sum_{i=1}^{q} \sum_{\forall s \in S} y_{\bar{e}ptis})\end{split}
\label{obj-1}
\end{equation}
Note that multiple solutions can yield the same value for $Max\_Slice\_Index$. To break the tie among multiple solutions, \eqn{obj-1} has a secondary objective of minimizing spectrum slice usage. The weight $\epsilon_2$ of the secondary objective function is chosen in a way that the second term is effective only when multiple solutions have same value for $Max\_Slice\_Index$.

%$\epsilon$ is chosen as a small constant, such that the second term is effective only when multiple solutions have the same value for the first part.
%\subsection{Complexity of the ILP}\label{subsec:hardness}
%Our formulation for the joint optimization problem has a quadratic constraint \eqn{cap_cons} and a quadratic objective function \eqn{obj}. Therefore, the QIP presented in \sect{subsec:qip} is a Quadratically Constrained Quadratic Program (QCQP) and falls into the general category of the Quadratic Assignment Problem (QAP)~\cite{lawler1963quadratic}. Solving a QAP is computationally  expensive and is known to be $\mathcal{NP}$-hard~\cite{cela2013quadratic}. Sahni \etal proved that even finding an $\epsilon-$approximate solution of QAP is NP-hard~\cite{sahni1976p}. In the next section, we present the steps to linearize the QIP by using a technique similar to the one discussed in~\cite{oral1992linearization}.
% and present the steps to  linearize our formulation in \sect{subsec:qip}.
% these two special problems to transform the quadratic objective function and quadratic constraint into a linear function and constraint, respectively.
\end{comment} 
